Temporal Relevance Analysis for Video Action Models

In this paper, we provide a deep analysis of temporal modeling for action recognition, an important but underexplored problem in the literature. We first propose a new approach to quantify the temporal relationships between frames captured by CNN-based action models based on layer-wise relevance propagation. We then conduct comprehensive experiments and in-depth analysis to provide a better understanding of how temporal modeling is affected by various factors such as dataset, network architecture, and input frames. With this, we further study some important questions for action recognition that lead to interesting findings. Our analysis shows that there is no strong correlation between temporal relevance and model performance; and action models tend to capture local temporal information, but less long-range dependencies. Our codes and models will be publicly available.

==> figures/fig_effect_backbones_new.tex <==
\begin{figure}[t]
	\centering
% 	\vspace{-2mm}
	\includegraphics[width=0.75\linewidth]{imgs/effect_datasets_v2.pdf}
	\vspace{-6mm}
	\caption{\small The effect of backbones on temporal relevance (16-frame models). The number on top of each bar indicates the number of temporal convolutions in a model while the number on the side is the model accuracy. This shows that avg-ATR does not correlate the strength of backbones. }
	\label{fig:effect_backbone_new}
\end{figure}


==> figures/fig_masking_exp_video_frame_rel.tex <==
\begin{figure}[t]
	\centering
% 	\vspace{-2mm}
	
	\begin{subfigure}{0.235\textwidth}
	\includegraphics[width=\linewidth]{imgs/top1_frame_video_rel_masking_kinetics.pdf}
	\caption{Top-1 Acc. on \Kinetics}
	\end{subfigure}
	\begin{subfigure}{0.235\textwidth}
	\includegraphics[width=\linewidth]{imgs/top5_frame_video_rel_masking_st2stv2.pdf}
    \caption{Top-5 Acc. on \Kinetics}
	\end{subfigure}
	\begin{subfigure}{0.235\textwidth}
	\includegraphics[width=\linewidth]{imgs/top1_frame_video_rel_masking_st2stv2.pdf}
	\caption{Top-1 Acc. on \SSV2}
	\end{subfigure}
	\begin{subfigure}{0.235\textwidth}
	\includegraphics[width=\linewidth]{imgs/top5_frame_video_rel_masking_st2stv2.pdf}
    \caption{Top-5 Acc. on \SSV2}
	\end{subfigure}
	\vspace{-3mm}
	\caption{Accuracy comparison by different number of input frames computed by frame-level temporal relevance and video-level temporal relevance. }
	\label{fig:masking_exp_video_frame_rel}
	\vspace{-2mm}
% 	\vspace{-2mm}
\end{figure}


==> figures/old_fig_effect_backbones.tex <==
% \begin{figure}[t]
% 	\centering
% % 	\vspace{-2mm}

%     \begin{subfigure}{0.235\textwidth}
%     \includegraphics[width=\linewidth]{imgs/effect_datasets.pdf}
% 	\caption{datasets}
% 	\end{subfigure}
	
% 	\begin{subfigure}{0.235\textwidth}
% 	\includegraphics[width=\linewidth]{imgs/effect_backbones_f16_only.pdf}
% 	\caption{\SSV2}
% 	\end{subfigure}
% 	\label{fig:effect_backbone}

% \end{figure}


==> figures/old_fig_inference_padding.tex <==
\begin{figure}[t]
	\centering
	\vspace{-2mm}
	\includegraphics[width=0.8\linewidth]{imgs/padding_inference.pdf}
	\vspace{-6mm}
	\caption{\small An illustration of ETRF verification by inference with padding. In this example, we use a f16 model and ETRF is 8. Given the frame $f_8$, we only use the frames within ETRF and replicated padding. }
	\label{fig:ragne_temporal}
	\vspace{-2mm}
\end{figure}
 

==> figures/old_fig_partial_uniform_sampling.tex <==
\begin{figure}[t]
	\centering
% 	\vspace{-2mm}
	\includegraphics[width=0.6\linewidth]{imgs/partial-uniform-sampling.pdf}
	\vspace{-3mm}
	\caption{\small  An illustration of partial uniform sampling. For a given frame $f$ (\eg $f_7$) in a window $W$ (\eg $f_4 - f_{11}$) from a set of uniformly sampled input frames, partial uniform sampling replaces the frames before $W$ by the start frame of $W$ (\ie $f_4$) and the frames after $W$ by the end frame of $W$ (\ie $f_{11}$). The modified input is fed into an action model to obtain the prediction for $f$. }
	\label{fig:partial-input-sampling}
	\vspace{-6mm}
\end{figure}


==> tables/ensemble_effects.tex <==

\begin{table}[t]
    \caption{\small Effects of frame ensemble. Models are trained with using different number of frames during prediction. Models are TAM-R50-16f on \SSV2.}
    \label{table:ensemble_effects}
    \centering
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{c|c|c}
        \toprule
        \# of frames & Ave. ETRF & Max. ETRF \\
        % \cmidrule{2-5}
        %              & Temporal       &  Static    & Temporal & Static \\
        \midrule
        1 & 8.67$\pm$0.81 & 8.67$\pm$0.81 \\
        2 & 7.68$\pm$0.91 & 8.64$\pm$0.92 \\
        4 & 7.18$\pm$0.56 & 7.93$\pm$0.61 \\
        8 & 6.99$\pm$0.49 & 7.90$\pm$0.66 \\
        16 & 7.22$\pm$0.50 & 8.25$\pm$0.70 \\
        
        % 1 & 8.67$\pm$0.81 & 8.67$\pm$0.81 \\
        % 2 & 6.11$\pm$1.58 & 8.65$\pm$0.97 \\
        % 4 & 6.86$\pm$0.76 & 7.97$\pm$0.75 \\
        % 8 & 6.71$\pm$0.60 & 7.98$\pm$0.87 \\
        % 16 & 6.96$\pm$0.61 & 8.34$\pm$0.93 \\
        % 1 & 7.26$\pm$0.20 & 12.03$\pm$0.28 \\
        % 2 & 7.27$\pm$0.46 & 15.00$\pm$0.21 \\
        % 4  & 7.27$\pm$0.52 & 9.55$\pm$2.57 \\
        % 8 & 7.15$\pm$0.64 & 9.21$\pm$0.78 \\ 
        % 16 & 6.96$\pm$0.61 & 8.34$\pm$0.93 \\
        \bottomrule
        % \multicolumn{8}{l}{\footnotesize{There is a performance of I3D and S3D from the original paper is b}}
    \end{tabular}
%    \vspace{-15pt}
    \end{adjustbox}
\end{table}

==> tables/temporal_analysis.tex <==

\begin{table}[t]
    \caption{\small The class overlap ratio, recognition accuracies and average temporal gains (in parenthesis) of the temporal and static datasets identified by human and machine}
    % \vspace{-2mm}
    \label{table:temporal_analysis}
%    \vspace{-8pt}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c}
        \toprule
             & \multicolumn{2}{c|}{SSV2} & \multicolumn{2}{c}{Kinetics}  \\
        \cmidrule{2-5}
                     & Temporal       &  Static    & Temporal & Static \\
        \midrule
        Class overlap ratio & 38.89\% &  11.11\% & 21.88\% & 3.12\% \\
        \midrule
        Human~\cite{temporal_dataset}   & 79.7\% (+47.8\%) & 71.1 (+31.7\%) & 75.0\% (+8.4\%) & 76.4\% (+8.2\%) \\
        Machine (Ours)    & 80.6\% (+68.9\%) & 83.4 (+24.7\%) & 73.5\% (+22.1\%) & 92.7\% (-1.7\%) \\
        \bottomrule
        % \multicolumn{8}{l}{\footnotesize{There is a performance of I3D and S3D from the original paper is b}}
    \end{tabular}
    }%resizebox
%    \vspace{-15pt}
\end{table}
